Bregman Power Divergences

Power distances between weighted Euclidean points are fundamental dissimilarity measures in computational geometry, used notably for constructing power diagrams and their dual weighted regular triangulations. Bregman divergences, on the other hand, are fundamental deviation measures in information theory and serve as canonical divergences of dually flat spaces in information geometry. In this work, we introduce Bregman power divergences, an extension of power distances to Bregman divergences, and provide two complementary geometric interpretations of that measure based on (i) the Bregman potential lifting and on (ii) the Bregman Pythagorean theorem. We show that Bregman power divergences between weighted parameters amount to equivalent ordinary power distances expressed using the mixed-parameterization induced by the convex duality of Bregman generators. This equivalence enables Bregman proximity problems to be solved as Euclidean proximity tasks at the expense of using an extra dimension. As an illustration of this equivalence, we reduce the Bregman diameter and closest-pair problems to Euclidean power distance problems. In the second part, we further elucidate the correspondence between Bregman power divergences and power distances through the equivalence of Bregman potential lifting and paraboloid lifting techniques. Last, we consider the space of Bregman and power spheres, and show how to construct a Bregman circumsphere passing through prescribed parameters as a corresponding power circumsphere, called an orthosphere. We further discuss several applications.

==> Fig/redundancyIT.tex <==
https://neurreps.org/
Information-theoretic minimax problems from the viewpoint of Laguerre geometry
Information-theoretic minimax problems made easy
fusion of probability mass functions

https://openreview.net/group?id=NeurIPS.cc/2025/Workshop/NeurReps#tab-accept-proceedings
https://neurips.cc/virtual/2025/loc/san-diego/workshop/109551
 


 



%%%%
\subsection{Smallest enclosing Bregman ball for universal coding}
%%%%


Source code with minimax redundancy is identical to the Chebyshev center problem with KL-divergence, capacity-redundancy [1, Ch. 13].


\def\KL{\mathrm{KL}}
\def\calX{\mathcal{X}}
\def\bbR{\mathbb{R}}

As an application of the smallest enclosing Bregman ball, consider the following  coding problem in information theory (chapter 13 of~\cite{ct-2012}, pp. 428-433):
Let $\calX=\{A_1, \ldots, A_d\}$ be a finite discrete alphabet of $d$ letters, and $X$ be a random variable with probability mass function $p$ on $\calX$.
Let $p_\lambda(x)$ denote the categorical distribution corresponding to $X$ (also called a multinoulli distribution) 
so that $\Pr(X=A_i)=p_\lambda(A_i)$ with $\lambda=(\lambda^1,\ldots,\lambda^d)\in\bbR_{++}^d$ and $\sum_{i=1}^d \lambda^i=1$.
The Huffman codeword for $x\in\calX$ is of length $l(x)=-\log p(x)$ (ignoring integer ceil rounding), 
and the expected codeword length of $X$ is thus given by Shannon's entropy $H(X)=-\sum_x p(x)\log p(x)$.
(Conversely, a codeword of length $l(x)$ has implied probability $2^{-l(x)}$.)
Now, if we code according to a distribution $p_{\lambda'}$ instead of the true distribution $p_\lambda$, the code is not optimal, and the {\em redundancy} $R(p_{\lambda},p_{\lambda'})$ is defined as 
the difference between the expected lengths of the codewords for $p_{\lambda'}$ and $p_{\lambda}$:
$$
R(p_{\lambda},p_{\lambda'})= (-E_{p_{\lambda}}[\log p_{\lambda'}(x)]  - (-E_{p_{\lambda}}[\log p_{\lambda}(x)]
= \KL(p_{\lambda}:p_{\lambda'})\geq 0,
$$
where KL stands for the Kullback-Leibler divergence.

Now, suppose that the true distribution $p_{\lambda}$ belong to one of $n$ prescribed distributions that we do not know: 
$p_\lambda \in \calP=\{p_{\lambda_1}, \ldots, p_{\lambda_n} \}$.
Then we seek for the minimax redundancy:
$$
R^*= \min_{p_{\lambda}} \max_{i\in \{1,\ldots, n\}} \KL(p_{\lambda_i}:p_{\lambda}).
$$
The distribution ${p_{\lambda^*}}$ achieving the minimax redundancy is the circumcenter of the KL ball enclosing the distributions $\calP$.
Using the natural coordinates $\theta=(\theta_1,\ldots,\theta_D)\in \bbR^D$ with $\theta_i=\log\frac{\lambda^i}{\lambda^d}$ of the categorical/multinoulli distributions (an exponential family of order $D=d-1$),
 we end up with calculating the smallest Bregman enclosing ball for the Bregman generator~\cite{EF-2009}: 
$F_{\mathrm{categorical}}(\theta)=\log (1+\sum_{i=1}^D \exp\theta_i)$:
$$
R^* = \min_{\theta\in \in \bbR^D} \max_{i\in [n]}  B_{F_{\mathrm{categorical}}}(p_\theta:p_{\theta_i}).
$$
This latter minimax problem is unconstrained since $\theta\in \in \bbR^D=\bbR^{d-1}$.

Remark. Figure 13.1 schematically draws a KL ball with 4 points on its boundary: 
It is a degenerate case since in general position (no $D+2$ lifted points $(\theta,F_{\mathrm{categorical}}(\theta))$ belonging to an hyperplane of $\bbR^{D+1}$, see~\ref{BVD-2010}) there are
$D+1$ points lying on the boundary of a Bregman ball.

